InternImage: Exploring Large-Scale Vision Foundation Models with Deformable Convolutions

Compared to the great progress of large-scale vision transformers (ViTs) in recent years, large-scale models based on convolutional neural networks (CNNs) are still in an early state. This work presents a new large-scale CNN-based foundation model, termed InternImage, which can obtain the gain from increasing parameters and training data like ViTs. Different from the recent CNNs that focus on large dense kernels, InternImage takes deformable convolution as the core operator, so that our model not only has the large effective receptive field required for downstream tasks such as detection and segmentation, but also has the adaptive spatial aggregation conditioned by input and task information. As a result, the proposed InternImage reduces the strict inductive bias of traditional CNNs and makes it possible to learn stronger and more robust patterns with large-scale parameters from massive data like ViTs. The effectiveness of our model is proven on challenging benchmarks including ImageNet, COCO, and ADE20K. It is worth mentioning that InternImage-H achieved a new record 65.4 mAP on COCO test-dev and 62.9 mIoU on ADE20K, outperforming current leading CNNs and ViTs. The code will be released at https://github.com/OpenGVLab/InternImage.

==> table_arxiv/ablation_msa.tex <==
\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.0}
    \setlength{\tabcolsep}{1.5mm}
    \footnotesize
    \begin{tabular}{c|cc|c|c}
    	\multirow{2}{*}{Divisor} & \multicolumn{2}{c}{IN-1k} & \#Param & FLOPs\\
    	& \scriptsize Top-1 & \scriptsize Top-5 & \scriptsize(M) & \scriptsize(G)\\
    	\whline
        1 &  &  &  & \\
        8 &  & &  & \\
        16 &  &  &  & \\
        32  &  &  & & \\
        \hline

    \end{tabular}
    \caption{\textbf{Ablation comparison of the group divisor $C'$.}
    }
    \label{tab:ablation_msa}
\end{table}

==> table_arxiv/det_cascade.tex <==
\begin{table}[t]\small
	\centering
	\renewcommand{\arraystretch}{0.93}
	\footnotesize
    \setlength\tabcolsep{2.4mm}{
    \begin{tabular}{l|cc|cccccc|cc}
        Method & \#Params & \#FLOPs & $\rm AP^b$ & $\rm AP^m$ \\
        \hline
        Swin-L$^\ddagger$~\cite{liu2021swin} & 253M & 1382G & 51.8 & 44.9  \\
        ConvNeXt-L$^\ddagger$~\cite{liu2022convnet} & 255M & 1354G & 53.5 & 46.4 \\
        \rowcolor{gray!20}
        \model-L$^\ddagger$ (ours) & 277M & 1399G & 54.9 & 47.7  \\
        \hline
        ConvNeXt-XL$^\ddagger$~\cite{liu2022convnet} & 407M & 1898G & 53.6 & 46.5 \\
        \rowcolor{gray!20}
        \model-XL$^\ddagger$ (ours) & 387M & 1782G & 55.3 & 48.0  \\
    \end{tabular}}
    
    \caption{
    \textbf{Object detection and instance segmentation with Cascade Mask R-CNN 1$\times$ schedule on COCO \texttt{val2017}.}
    The FLOPs are measured with 1280$\times$800 inputs.
	}
    \label{tab:results_detection_cascade}
    \label{tab:mask}
\end{table}

==> table_arxiv/model_size.tex <==
\begin{tabular}{l|c|c|c|c}
    \renewcommand{\arraystretch}{0.1}
	Model Name & $C$ & \#Blocks  & \#Groups & \#P (M) \\
	\hline
        \model-T &64 &(4, 4, 18, 4) & (4, 8, 16, 32) & 29 \\
        \model-S &80 &(4, 4, 21, 4) & (5, 10, 20, 40) & 50 \\
        \model-B &112 &(4, 4, 21, 4) & (7, 14, 28, 56) & 97 \\
        \model-L &160 &(5, 5, 22, 5) & (10, 20, 40, 80) & 223 \\
        \model-XL &160 &(5, 5, 24, 5) & (12, 24, 48, 96) & 335 \\
        \model-H &320 &(6, 6, 32, 6) & (20, 40, 80, 160) & 1000
\end{tabular}

==> table_arxiv/seg_sota.tex <==
\begin{table}[t]\small
	\centering
	\renewcommand{\arraystretch}{0.95}
	\footnotesize
    \setlength\tabcolsep{0.4mm}{
    \begin{tabular}{l|l|c|cc}
        \multirow{2}{*}{Method} & \multirow{2}{*}{Detector} & \multirow{2}{*}{\#Params} & \multicolumn{2}{c}{box AP} \\
        &  & & val2017 & test-dev \\
	    \hline
	Swin-L$^\ddagger$~\cite{liu2021swin} 
	& HTC++~\cite{liu2021swin} & 284M & 58.0 & 58.7 \\
	    
        
        ViT-Adapter-L$^\ddagger$~\cite{chen2022vitadapter} 
        & HTC++~\cite{liu2021swin} & 401M & 60.5 & 60.9 \\
        
        Swin-L$^\ddagger$~\cite{liu2021swin} 
        & Soft-Teacher~\cite{xu2021end} & 284M & 60.7 & 61.3 \\
        
        Swin-L$^\ddagger$~\cite{liu2021swin} 
        & DINO~\cite{zhang2022dino} & 218M & 63.2 & 63.3 \\

        \hline
        
        Florence-CoSwin-H$^\#$~\cite{yuan2021florence} 
        & DyHead~\cite{dai2021dynamic} & 
        637M
        & 62.0 & 62.4 \\
        
        SwinV2-G~$^\#$\cite{liu2021swinv2} 
        & HTC++~\cite{liu2021swin} & 3.00B & 62.5 & 63.1 \\
        
        BEiT-3$^\#$~\cite{wang2022beit3} 
        & ViTDet~\cite{li2022exploring} & 1.90B &$-$ & 63.7 \\
        
        FD-SwinV2-G$^\#$~\cite{wei2022fdswin}
        & HTC++~\cite{liu2021swin} & 3.00B & $-$ & 64.2 \\
        
        
        \hline
        \rowcolor{gray!10}
        \model-XL$^\ddagger$ (ours) 
        & DINO~\cite{zhang2022dino} & 602M & 64.2 & 64.3 \\ 
        \rowcolor{gray!20}
        \model-H$^\#$ (ours) 
        & DINO~\cite{zhang2022dino} & 2.18B & 65.0 & 65.3\\
    \end{tabular}
    }
    \vspace{0.05cm}
    \caption{\textbf{Comparison of the state-of-the-art segmenters on ADE20K valiation set.} 
    }
    \label{tab:seg_sota}
\end{table}

==> table_arxiv/supp_det_setting.tex <==
\begin{tabular}{l|ccc|cc|c}
    \renewcommand{\arraystretch}{0.1}
    \setlength\tabcolsep{0.97mm}
    settings & T & S & B & L & XL & H \\
    \hline
    Pre-training & \multicolumn{3}{c|}{IN-1K} & \multicolumn{2}{c|}{IN-22K} & O365 \\ 
    Detector & \multicolumn{3}{c|}{Mask R-CNN} & \multicolumn{2}{c|}{Cascade.} & DINO \\
    \hline
    Optimizer & \multicolumn{3}{c|}{AdamW} & \multicolumn{2}{c|}{AdamW} & AdamW \\
    LR & \multicolumn{3}{c|}{1e-4} & \multicolumn{2}{c|}{1e-4} & 1e-4 \\
    Layer-wise LR & \multicolumn{3}{c|}{1.0} & \multicolumn{2}{c|}{0.9} & 0.94 \\
    Train Epochs & \multicolumn{3}{c|}{36} & \multicolumn{2}{c|}{36} & 12 \\
    Drop Path    & 0.2 & 0.4 & 0.5 & 0.5 & 0.6 & 0.5 \\
    Batch Size & \multicolumn{3}{c|}{16} & \multicolumn{2}{c|}{16} & 64 \\
    Weight Decay & \multicolumn{3}{c|}{0.05} & \multicolumn{2}{c|}{0.05} & 0.0001 \\
    EMA & \multicolumn{3}{c|}{\no} & \multicolumn{2}{c|}{\no} & \no \\
    
\end{tabular}

==> table_arxiv/supp_tensorrt.tex <==
\begin{tabular}{l|c|c|c}
    \multirow{2}{*}{method} & \multicolumn{3}{|c|}{batch size} \\
     & 128 & 32 & 12\\
    \hline
    \model-T & 1.22 & 4.81 & 18.87 \\
    \model-S & 1.70 & 6.76 & 26.32 \\
    \model-B & 2.39 & 9.43 & 37.04 \\
\end{tabular}

==> table_arxiv/supp_tiny_setting.tex <==
\begin{tabular}{c|c}
    \renewcommand{\arraystretch}{0.1}
    \setlength\tabcolsep{0.97mm}
    configuration & value \\
    \hline
    optimizer & AdamW \\
    base learning rate & 5e-4 \\
    warmup learning rate & 5e-7 \\
    learning rate schedule & cosine decay \\
    train epochs & 300 \\
    warmup epochs & 20 \\
    batch size & 4096 \\
    weight decay & 0.05 \\
    EMA decay & 0.9999 \\
    input size  & $224\times224$ \\
    kernel size & $3\times3$ \\
    normalization type & LN \\
    MLP ratio & 4.0 \\
    drop path rate & 0.1 \\
    mix up & 0.8 \\
    cut mix & 1.0 \\
    color jitter & 0.4 \\
\end{tabular}
